Search for FCNC in top quark production and decays

An overview of searches for top quark flavour changing neutral currents (FCNC) from the CDF, D0, ATLAS and CMS collaborations is presented. The FCNC interactions of top quarks are probed through the anomalous decays and production channels. No clear evidence for the presence of the signal is observed in none of the searches and the upper limits are set at 95% confidence level (CL) on the cross sections, anomalous couplings and the branching ratios.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = smith_joe

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}
	

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg \
              *.inx *.dvi *.toc *.out *~ ~* */*~ */~* spellTmp 

